Found in Translation: Measuring Multilingual LLM Consistency as Simple as Translate then Evaluate

Large language models (LLMs) provide detailed and impressive responses to queries in English. However, are they really consistent at responding to the same query in other languages? The popular way of evaluating for multilingual performance of LLMs requires expensive-to-collect annotated datasets. Further, evaluating for tasks like open-ended generation, where multiple correct answers may exist, is nontrivial. Instead, we propose to evaluate the predictability of model response across different languages. In this work, we propose a framework to evaluate LLM's cross-lingual consistency based on a simple Translate then Evaluate strategy. We instantiate this evaluation framework along two dimensions of consistency: information and empathy. Our results reveal pronounced inconsistencies in popular LLM responses across thirty languages, with severe performance deficits in certain language families and scripts, underscoring critical weaknesses in their multilingual capabilities. These findings necessitate cross-lingual evaluations that are consistent along multiple dimensions. We invite practitioners to use our framework for future multilingual LLM benchmarking.

==> sections/framework.tex <==
\section{A Framework for Cross-lingual Consistency}
\label{sec:framework}
Evaluating cross-lingual consistency of LLMs is uniquely challenging, especially for open-ended or nuanced tasks where standard accuracy metrics are inapplicable. A key obstacle is that most modern evaluators---be it for factuality, empathy, or even coherence---are monolingual and validated primarily on English data. Multilingual evaluation is either unreliable or infeasible in the absence of high-quality resources for other languages.

We address this challenge via a general and scalable framework for measuring cross-lingual consistency, centered around a simple yet effective principle: \textit{Translate then Evaluate}.\footnote{This approach is similar to the widely used and highly effective baseline of translating the input before answering, as noted in~\citet{shilanguage}.\vs{Missing year in bib entry}} This paradigm allows us to exploit well-established English-language evaluation pipelines, extending their utility to a much broader set of languages.

Let us formalize this idea. 
We begin by defining the notion of an evaluator. An evaluator $\mathcal{E}$ is a function that takes two text inputs \vs{in the same language? Or not necessarily?} and returns a compatibility score.  Evaluators may be based on traditional heuristic metrics, such as BLEU or ROUGE, which compute n-gram overlap, or on more recent LLM-based methods like FActScore~\citep{min2023factscore} and VeriScore~\citep{song2024veriscore}. 
% In general, $\mathcal{E}$ maps a text pair to a scalar score representing their alignment.



Let $\mathcal{X}$ denote a set of prompts, where each prompt $x \in \mathcal{X}$ may be expressed in any language $\ell \in \mathcal{L}$, with English denoted by $\texttt{en}$. We denote the translation of the prompt $x$ in language $\ell$ as $x_{\ell}$, and its English version as $x_{\text{en}}$. 
%
\vs{There is a subtle confusion between the first two sentences. Sentence 1 says $x$ can be in any language. Sentence 2 says that $x_\ell$ is the translation of $x$ to $\ell$. What is it being translated from? Is $x_\ell$ in $\mathcal{X}$? Should we think of $\mathcal{X}$ as being partitioned by language? Or is $\mathcal{X}$ just a set of prompts in whatever language, and we translate every prompt to every language (as sentence 2 may be interpreted)?} \vs{After reading the whole thing, I am even more confused about what $x$'s language is.}
\ag{Let $\mathcal{X}$ denote a set of abstract prompts, where each prompt $x \in \mathcal{X}$ represents a language-agnostic intent or input (e.g., a question or instruction). For any language $\ell \in \mathcal{L}$, we denote by $x_\ell$ the realization of $x$ in language $\ell$, with English denoted by $\texttt{en}$. In particular, $x_{\texttt{en}}$ refers to the English version of $x$. Does this work?}\mm{Don't like the word 'abstract' here }\vs{I don't like 'abstract' either.}
\mm{Let $\mathcal{X}$ denote a set of prompts. Each $x$ in $\mathcal{X}$ can be translated to a language $\ell \in \mathcal{L}$ independent of the prompt's source language. We denote each of these prompts in language $\ell$ as $x_{\ell}$}
%
Additionally, for a given multilingual LLM $\mathcal{M}$, we define its generated response to prompt $x$ in language $\ell$ as:
\begin{align}
r_{\ell}(x) = \mathcal{M}(x_{\ell}).
\end{align}

We define consistency $\mathcal{C}$ as the compatibility score computed by an evaluator $\mathcal{E}$ between the English response and non-English response, $r_{\text{en}}(x)$ and $r_{\ell}(x)$ as:
\begin{align}
\mathcal{C}_{\mathcal{M}, \mathcal{E}}(x, \ell) = \mathcal{E}\left( r_{\text{en}}(x), r_{\ell}(x) \right)
\end{align}

\vs{Just noticed an oddity here. We have script fonts (with mathcal) for sets ($\mathcal{X}, \mathcal{L}$), for programs ($\mathcal{M}$) and for functions ($\mathcal{C}, \mathcal{E}$). It can be a bit much. Suggestion: Use script font only for sets. Let the evaluator and consistency, and the model can be typewriter font. Maybe evaluator and consistency are in lower case. May be easiest to make macros for these.}

\vs{Alternate version (see last notes below): 
We define consistency $\mathcal{C}$ as the expected compatibility score computed by an evaluator $\mathcal{E}$ between the English response and non-English response, $r_{\text{en}}(x)$ and $r_{\ell}(x)$. The expectation is computed over prompts $x$, giving us:
\begin{align}
\mathcal{C}_{\mathcal{M}, \mathcal{E}}(\ell) = \mathbb{E}_{x}\left[\mathcal{E}\left(r_{\text{en}}(x), r_{\ell}(x) \right)\right]
\end{align}
}

Directly comparing $r_{\text{en}}(x)$ and $r_{\ell}(x)$ is non-trivial\mm{We can cite alignment literature here}, particularly because most model-based evaluators are monolingual and optimized for English. To resolve this, we use a translation model $\mathcal{T}_{\ell \rightarrow {\text{en}}}$ that maps responses from the target language $\ell$ to English:
\begin{align}
\hat{r}_{\ell \rightarrow \text{en}}(x) = \mathcal{T}_{\ell \rightarrow {\text{en}}}(r_{\ell}(x)).
\end{align}
\mm{Why don't we simplify and just right it as $\hat{r}_{\ell}(x)$}\vs{Yes}

This translation brings both responses into a common language, enabling the use of English-only evaluators. 
% We can now apply any downstream evaluator $\mathcal{E}$ designed for English by 
Substituting non-English response $r_{\ell}(x)$ with its corresponding English translation $\hat{r}_{\ell \rightarrow \text{en}}(x)$ and we redefine consistency as:
\begin{align}
\mathcal{C}_{\mathcal{M}, \mathcal{E}}(x, \ell) = \mathcal{E}\left( r_{\text{en}}(x), \hat{r}_{\ell \rightarrow \text{en}}(x) \right)
\end{align}

\vs{shouldnt the $=$ be $\approx$ above? Equality is a bit too strong to ask for}

\vs{Alternate version: \\
Under the assumption that $\mathcal{E}$ produces the \textit{similar} scores before and after translation, we can approximate consistency as:
\begin{align}
\mathcal{C}_{\mathcal{M}, \mathcal{E}}(\ell) \approx \mathbb{E}_x\left[\mathcal{E}\left( r_{\text{en}}(x), \hat{r}_{\ell \rightarrow \text{en}}(x) \right)\right]
\end{align}
}

Under the assumption that $\mathcal{E}$ produces the \textit{similar} scores before and after translation:
\begin{align}
\mathcal{E}\left( r_{\text{en}}(x), r_{\ell}(x) \right) = \mathcal{E}\left( r_{\text{en}}(x), \hat{r}_{\ell \rightarrow \text{en}}(x) \right)
\end{align}
\mm{It should be an approximation and not an equality}\vs{Yes. See above too.}
\vs{In the alternate version, we won't need the above para}

Finally, the consistency \vs{of the model $\mathcal{M}$ for language $\ell$ with respect to an evalator $\mathcal{E}$}, denoted by $\mathcal{C}_{\mathcal{M}, \mathcal{E}}(\ell)$, is obtained by averaging over the set of prompts $x \in \mathcal{X}$ as:
\begin{align}
\mathcal{C}_{\mathcal{M}, \mathcal{E}}(\ell) = \frac{1}{|\mathcal{X}|} \sum_{x \in \mathcal{X}} \mathcal{E}\left( r_{\text{en}}(x), \hat{r}_{\ell \rightarrow \text{en}}(x) \right)
\end{align}

\vs{Alternate version:\\
In practice, of course, we cannot compute the expectation over all possible inputs $x$, and instead approximate the consistency as the empirical mean over a set of prompts $x \in \mathcal{X}$:
\begin{align}
\mathcal{C}_{\mathcal{M}, \mathcal{E}}(\ell) \approx \frac{1}{|\mathcal{X}|} \sum_{x \in \mathcal{X}} \mathcal{E}\left( r_{\text{en}}(x), \hat{r}_{\ell \rightarrow \text{en}}(x) \right)
\end{align}}


\vs{I have an idea to make the notation a bit cleaner. Let us never define consistency for a specific input (i.e. $x$ is never an argument for the consistency). Instead, let us define consistency as \emph{expected} evaluator score. See alternate versions I have interleaved below.}\mm{I like the alternative framework}

\paragraph{Desideratum for the Translation Model.} 
As noted above, a critical requirement of this framework is that the translation model $\mathcal{T}$ preserves the semantic and pragmatic properties that the evaluator $\mathcal{E}$ is designed to measure. In our experiments, we employ the state-of-the-art NLLB 54B-parameter Mixture-of-Experts (MoE) model~\cite{costa2022no}, which has demonstrated superior performance over conventional systems such as Google Translate for English-targeted translation across a wide range of languages.
% As mentioned above, a critical requirement for this framework is that the translation system $\mathcal{T}$ preserves the underlying property the evaluator $\mathcal{E}$ tries to capture. In practice, we use the state-of-the-art NLLB 54B-parameter Mixture-of-Experts (MoE) translation model~\cite{costa2022no}, which has been shown to outperform conventional systems like Google Translate for English-targeted translation across a wide variety of languages. 

\paragraph{Discussion.} 
% To understand the consistency of multilingual LLMs, we need to use different kinds of evaluators. 
% Our framework can be applied with any off-the-shelf evaluator that works well in English.
% Ideally, we need a large collection of evaluators to study multilingual performance profiles of LLMs, each of them developed to understand consistency of targeted properties. In this work, we instantiate this framework for two off-the-shelf (readily available) evaluators targeting two different properties:
% The evaluator $\mathcal{E}$ can directly take a pair of texts and produce a score comparing the two texts (like FActScore). It can also take a property (say, sentiment), compute it separately for the pair of texts, and then produce a score comparing the property.
To evaluate the consistency of multilingual LLMs, it is essential to employ diverse types of evaluators. Our proposed framework is agnostic to this choice and can be instantiated with any English-capable evaluator\mm{Or a combination of them?? Remember, the psychotherapy evaluator is a combination of three sub-evaluators. We might want to make this point independently. I think the next line alludes to this a bit but we need to state that they can combine to form "an" evaluator}. Ideally, a broad suite of evaluators---each targeting a specific linguistic or functional property---will help characterize the multilingual performance profiles of LLMs. The evaluator itself may operate in one of the two modes. In the first, it can directly compare a pair of texts to produce a similarity or compatibility score similar to FActScore. In the second mode, it can target a specific property (e.g., sentiment), compute this property independently for each text, and then compare the resulting attributes to derive a score. 
In this work, we instantiate our framework using two readily available, off-the-shelf evaluators operating in these two modes. We will discuss these in the next section.
\section{Instantiations of Cross-Lingual Consistency}
\input{tables/human_eval_info_scores}

==> sections/methodology.tex <==
\section{Methodology}
We instantiate our \discrepancy~framework with three tasks: open-ended generation, empathy in mental health, and situations of moral dilemma. 


==> sections/todo.tex <==
\section{TODO}

\begin{enumerate}
    \item Factor Analysis
    \item To Indic or not to Indic
    \item Human validation for a) open-ended b) psychotherapy
    \item Human error analysis on best performing model,languages (sort by increasing F1 scores) 
    --- Frame it as error analysis vs annotation (authors can't do this)
    
\end{enumerate}


-- Cite following papers:

\begin{enumerate}
    \item Morality across languages in LLMs~\citep{khandelwal2024moral}
    \item 
\end{enumerate}
